Mirage-1: Augmenting and Updating GUI Agent with Hierarchical Multimodal Skills

Recent efforts to leverage the Multi-modal Large Language Model (MLLM) as GUI agents have yielded promising outcomes. However, these agents still struggle with long-horizon tasks in online environments, primarily due to insufficient knowledge and the inherent gap between offline and online domains. In this paper, inspired by how humans generalize knowledge in open-ended environments, we propose a Hierarchical Multimodal Skills (HMS) module to tackle the issue of insufficient knowledge. It progressively abstracts trajectories into execution skills, core skills, and ultimately meta-skills, providing a hierarchical knowledge structure for long-horizon task planning. To bridge the domain gap, we propose the Skill-Augmented Monte Carlo Tree Search (SA-MCTS) algorithm, which efficiently leverages skills acquired in offline environments to reduce the action search space during online tree exploration. Building on HMS, we propose Mirage-1, a multimodal, cross-platform, plug-and-play GUI agent. To validate the performance of Mirage-1 in real-world long-horizon scenarios, we constructed a new benchmark, AndroidLH. Experimental results show that Mirage-1 outperforms previous agents by 32\%, 19\%, 15\%, and 79\% on AndroidWorld, MobileMiniWob++, Mind2Web-Live, and AndroidLH, respectively. Project page: https://cybertronagent.github.io/Mirage-1.github.io/

==> figures/ablation_study.tex <==
\begin{figure}[ht]
\centering
\includegraphics[width=0.4\textwidth]{figures/chart.pdf}
\caption{We compared three online exploration methods: direct exploration, MCTS, and SA-MCTS on $30$ \texttt{GPT-4o} generated tasks. Results show that SA-MCTS acquires more skills than the other methods, demonstrating its superior effectiveness in online exploration.}
\label{abl-mcts}
\end{figure}

==> figures/intro.tex <==
\begin{figure*}[ht]
    \centering
    \includegraphics[width=1\textwidth]{figures/fig1.pdf}
    \caption{Comparison between existing GUI Agents and ours. Existing GUI agents exhibit significant limitations in executing long-horizon tasks and lack generalization ability. In contrast, Mirage delivers a performance boost by: (1) a \textbf{Hierarchical Multimodal Skills} (HMS) module that enhances the agent's capability in long-horizon task planning, and (2) a \textbf{Skill-Augmented MCTS} algorithm that leverages the HMS to search feasible trajectories in online environments.}
    \label{fig-intro}
\end{figure*}

==> tables/android_world.tex <==
% \begin{table*}[t]\small
% \centering
% \begin{tabular}{clllcc}
% \toprule[1.5pt]
% \textbf{Method} & \textbf{Input} &\textbf{Planner} & \textbf{Operator} & \textbf{AndroidWorld} & \textbf{MobileMiniWob++} \\ 
% \midrule
%  \multirow{5}{*}{\citealp{rawles2024androidworld}} & \multirow{2}{*}{AXTree}  & GPT-4-Turbo & \multirow{2}{*}{Choice} & 30.6 & 59.7 \\
% & &  Gemini 1.5 Pro &  & 19.4 & 57.4 \\ 
% \midrule
% & \multirow{3}{*}{Image+AXTree} 
%  & GPT-4-Turbo & \multirow{3}{*}{SoM} & 25.4 & 67.7 \\
% & & Gemini 1.5 Pro &  & 22.8 & 40.3 \\
% & & SeeAct &  & 15.5 & 66.1 \\ 
% \midrule

% & \multirow{6}{*}{Image} & GPT-4o & OS-Atlas & 31.9$^*$ & 51.1$^*$ \\
% \rowcolor[HTML]{E7EEFE}
% \cellcolor{white} &  \cellcolor{white} & Mirage & OS-Atlas & \textbf{42.2} & \textbf{60.9} \\ \cmidrule{3-6} 
% & & GPT-4o & UGround & 32.8 & 48.4 \\
% \rowcolor[HTML]{E7EEFE}
% \cellcolor{white} & \cellcolor{white} & Mirage & UGround & \textbf{40.5} & \textbf{56.5} \\ \cmidrule{3-6} 
% & & GPT-4o & Aria-UI & 37.1$^*$ & 52.2$^*$ \\
% \rowcolor[HTML]{E7EEFE}
% \cellcolor{white}& \cellcolor{white} & Mirage & Aria-UI & \textbf{41.4} & \textbf{62.0} \\ 
% \bottomrule[1.5pt]
% \end{tabular}
% \caption{\label{android_wrold_result}
% Performance comparison on AndroidWorld and MobileMiniWob++. We report task success rate (SR). $^*$ means the results reproduced by ourselves under the same prompt setting.
% }
% \end{table*}


% \begin{table*}[t]\small
% \centering
% \begin{tabular}{l|llcc}
% \toprule[1.5pt]
% \multicolumn{1}{l|}{\textbf{Method}} & \multicolumn{1}{l}{\textbf{Planner}} & \textbf{Operator} & \textbf{AndroidWorld$_{SR}$} & \textbf{MobileMiniWob++$_{SR}$} \\
% \midrule
%  & \multicolumn{4}{c}{\textbf{AXTree}} \\ \midrule
% \multicolumn{1}{c|}{\multirow{2}{*}{\citeauthor{rawles2024androidworld}}} & GPT-4-Turbo & \multirow{2}{*}{Choice} & 30.6 & 59.7 \\
% \multicolumn{1}{c|}{} & Gemini 1.5 Pro &  & 19.4 & 57.4 \\ \midrule
% \multicolumn{1}{c|}{} & \multicolumn{4}{c}{\textbf{Image + AXTree}} \\ \midrule
% \multirow{3}{*}{\citeauthor{rawles2024androidworld}} & GPT-4-Turbo & \multirow{3}{*}{SoM} & 25.4 & 67.7 \\
%  & Gemini 1.5 Pro &  & 22.8 & 40.3 \\
%  & SeeAct &  & 15.5 & 66.4 \\ \midrule
%  & \multicolumn{4}{c}{\textbf{Image}} \\ \midrule
% \citeauthor{wu2024osatlas} & GPT-4o & OS-Atlas & 31.9$^*$ & 51.1$^*$ \\\rowcolor[HTML]{E7EEFE}
% Mirage-O & GPT-4o & OS-Atlas & \textbf{42.2} & \textbf{60.9} \\
% \multirow{2}{*}{\citeauthor{gou2024uground}} & GPT-4-Turbo & UGround & 31.0 & - \\
%  & GPT-4o & UGround & 32.8$^*$ & 48.4$^*$ \\
% \rowcolor[HTML]{E7EEFE}
% Mirage-U & GPT-4o & UGround & \textbf{40.5} & \textbf{56.5} \\
% \citeauthor{yang2024aria-ui} & GPT-4o & Aria-UI & 37.1$^*$ & 52.2$^*$ \\\rowcolor[HTML]{E7EEFE}
% Mirage-A & GPT-4o & Aria-UI & \textbf{41.4} & \textbf{62.0} \\ \bottomrule[1.5pt]
% \end{tabular}
% \caption{\label{android_wrold_result}
% Performance comparison on AndroidWorld and MobileMiniWob++. We report task success rate (SR). $^*$ means the results reproduced by ourselves under the same prompt setting.
% }
% \end{table*}

\begin{table*}[t]\small
\centering
\begin{tabular}{l|cll}
\toprule[1.5pt]
\multicolumn{1}{l|}{\textbf{Method}} & \textbf{Operator} & \textbf{AndroidWorld} & \textbf{MobileMiniWob++} \\
\midrule
 & \multicolumn{3}{c}{\textbf{AXTree}} \\ \midrule
\multicolumn{1}{c|}{\multirow{2}{*}{\citeauthor{rawles2024androidworld}}} & GPT-4-Turbo +   Choice & 30.6 & 59.7 \\
\multicolumn{1}{c|}{} & Gemini 1.5 Pro  + Choice   & 19.4 & 57.4 \\ \midrule
\multicolumn{1}{c|}{} & \multicolumn{3}{c}{\textbf{Image + AXTree}} \\ \midrule
\multirow{3}{*}{\citeauthor{rawles2024androidworld}} & GPT-4-Turbo + SoM & 25.4 & 67.7 \\
 & Gemini 1.5 Pro  + SoM  & 22.8 & 40.3 \\
 & SeeAct  + SoM  & 15.5 & 66.4 \\ \midrule
 & \multicolumn{3}{c}{\textbf{Image}} \\ \midrule
\citeauthor{wu2024osatlas} & GPT-4o + OS-Atlas & 31.9$^*$ & 51.1$^*$ \\\rowcolor[HTML]{E7EEFE}
Mirage-O & GPT-4o + OS-Atlas & \textbf{42.2}$_{\color{teal}{\textbf{\scriptsize32.3\%}\uparrow}}$ & \textbf{60.9}$_{\color{teal}{\textbf{\scriptsize19.1\%}\uparrow}}$ \\
\multirow{2}{*}{\citeauthor{gou2024uground}} & GPT-4-Turbo + UGround & 31.0 & - \\
 & GPT-4o + UGround & 32.8$^*$ & 48.4$^*$ \\
\rowcolor[HTML]{E7EEFE}
Mirage-U & GPT-4o + UGround & \textbf{40.5}$_{\color{teal}{\textbf{\scriptsize23.4\%}\uparrow}}$ & \textbf{56.5}$_{\color{teal}{\textbf{\scriptsize16.7\%}\uparrow}}$ \\
\citeauthor{yang2024aria-ui} & GPT-4o + Aria-UI & 37.1$^*$ & 52.2$^*$ \\\rowcolor[HTML]{E7EEFE}
Mirage-A & GPT-4o + Aria-UI & \textbf{41.4}$_{\color{teal}{\textbf{\scriptsize11.6\%}\uparrow}}$ & \textbf{62.0}$_{\color{teal}{\textbf{\scriptsize18.8\%}\uparrow}}$ \\ \bottomrule[1.5pt]
\end{tabular}
\caption{\label{android_wrold_result}
Performance comparison on AndroidWorld and MobileMiniWob++. We report task success rate (SR). $^*$ means the results reproduced by ourselves under the same prompt setting.
}
\end{table*}

==> tables/long_horizon.tex <==
% \begin{table*}\small
% \centering
% \begin{tabular}{clllcc}
% \toprule[1.5pt]
% \textbf{Inputs} & \textbf{Agent} & \textbf{Operator} & \textbf{Grounding} & \textbf{Completion Rate} & \textbf{Success Rate} \\ \midrule
% AXTree & M3A & GPT-4o & Choice & 38.1 & 20.0  \\ \midrule
% \multirow{2}{*}{Image+AXTree} & M3A & GPT-4o & \multirow{2}{*}{SoM} & 31.7 & 23.3 \\
%  & SeeAct & GPT-4o &  & 30.2  & 13.3 \\ \midrule
% \multirow{6}{*}{Image} & M3A & \multirow{2}{*}{GPT-4o} & \multirow{2}{*}{OS-Atlas} & 27.0  & 16.7  \\
%  & Mirage &  &  & \textbf{50.8} & \textbf{30.0} \\ \cline{2-6} 
%  & M3A & \multirow{2}{*}{GPT-4o} & \multirow{2}{*}{UGround} & 39.7  & 26.7 \\
%  & Mirage &  &  & \textbf{55.6} & \textbf{36.7} \\ \cline{2-6} 
%  & M3A & \multirow{2}{*}{GPT-4o} & \multirow{2}{*}{Aria-UI} & 31.7 & 23.3  \\
%  & Mirage &  &  & \textbf{49.2} & \textbf{36.7} \\ \bottomrule[1.5pt]
% \end{tabular}
% \caption{\label{long_horizon_result}
% Performance comparison on Mobile-Long. We report completion rate (CR) and task success rate (SR).
% }
% \end{table*}

% \begin{table}\small
% \centering
% \begin{tabular}{l|llcc}
% \toprule[1.5pt]
% \textbf{Method}  & \textbf{Planner} & \textbf{Operator} & \textbf{CR} & \textbf{SR} \\ 
% \midrule
% & \multicolumn{4}{c}{\textbf{AXTree}} \\ \midrule
% \citeauthor{rawles2024androidworld} & GPT-4o & Choice & 38.1 & 20.0  \\ \midrule
% & \multicolumn{4}{c}{\textbf{Image + AXTree}} \\ \midrule
% \citeauthor{rawles2024androidworld}  & GPT-4o & \multirow{2}{*}{SoM} & 31.7 & 23.3 \\
% \citeauthor{zheng2024seeact}  & GPT-4-Turbo &  & 30.2  & 13.3 \\ 
%   \midrule
%   & \multicolumn{4}{c}{\textbf{Image}} \\ \midrule
% \citeauthor{wu2024osatlas}  & GPT-4o & OS-Atlas & 27.0  & 16.7  \\
% \rowcolor[HTML]{E7EEFE}
% Mirage-O & GPT-4o  & OS-Atlas  & \textbf{50.8} & \textbf{30.0} \\ 
%  \citeauthor{gou2024uground} & GPT-4o & UGround & 39.7  & 26.7 \\
%  \rowcolor[HTML]{E7EEFE}
% Mirage-U &  GPT-4o  & UGround & \textbf{55.6} & \textbf{36.7} \\ 
%  \citeauthor{yang2024aria-ui} & GPT-4o & Aria-UI & 31.7 & 23.3  \\
%  \rowcolor[HTML]{E7EEFE}
%  Mirage-A & GPT-4o  & Aria-UI & \textbf{49.2} & \textbf{36.7} \\ 
% \bottomrule[1.5pt]
% \end{tabular}
% \caption{\label{long_horizon_result}
% Performance comparison on AndroidLH. We report completion rate (CR) and task success rate (SR).
% }
% \end{table}

\begin{table}\small
\centering
\begin{tabular}{l|cll}
\toprule[1.5pt]
\textbf{Method}  &  \textbf{Operator} & \textbf{CR} & \textbf{SR} \\ 
\midrule
& \multicolumn{3}{c}{\textbf{AXTree}} \\ \midrule
\citeauthor{rawles2024androidworld} & GPT-4o + Choice & 38.1 & 20.0  \\ \midrule
& \multicolumn{3}{c}{\textbf{Image + AXTree}} \\ \midrule
\citeauthor{rawles2024androidworld}  & GPT-4o + SoM & 31.7 & 23.3 \\
\citeauthor{zheng2024seeact}  & GPT-4-Turbo + SoM  & 30.2  & 13.3 \\ 
  \midrule
  & \multicolumn{3}{c}{\textbf{Image}} \\ \midrule
\citeauthor{wu2024osatlas}  & GPT-4o + OS-Atlas & 27.0  & 16.7  \\
\rowcolor[HTML]{E7EEFE}
Mirage-O & GPT-4o  + OS-Atlas  & \textbf{50.8} & \textbf{30.0}$_{\color{teal}{\textbf{\scriptsize79.6\%}\uparrow}}$ \\ 
 \citeauthor{gou2024uground} & GPT-4o + UGround & 39.7  & 26.7 \\
 \rowcolor[HTML]{E7EEFE}
Mirage-U &  GPT-4o  + UGround & \textbf{55.6} & \textbf{36.7}$_{\color{teal}{\textbf{\scriptsize37.4\%}\uparrow}}$ \\ 
 \citeauthor{yang2024aria-ui} & GPT-4o + Aria-UI & 31.7 & 23.3  \\
 \rowcolor[HTML]{E7EEFE}
 Mirage-A & GPT-4o  + Aria-UI & \textbf{49.2} & \textbf{36.7}$_{\color{teal}{\textbf{\scriptsize57.5\%}\uparrow}}$ \\ 
\bottomrule[1.5pt]
\end{tabular}
\caption{\label{long_horizon_result}
Performance comparison on AndroidLH. We report completion rate (CR) and task success rate (SR).
}
\end{table}

==> tables/mcts_ablation.tex <==
\begin{table}\small
\centering
\begin{tabular}{lc}
\toprule[1.5pt]
Method & \multicolumn{1}{c}{Skill Number $\uparrow$ } \\ \midrule
Direct & 6  \\
MCTS &  12 \\
\rowcolor[HTML]{E7EEFE}
Skill-Augmented MCTS & \textbf{17} \\ \bottomrule[1.5pt]
\end{tabular}
\caption{\label{abl-mcts}
Ablation study to evaluate the effectiveness of various online exploration methodologies. We utilized $30$ Android tasks generated via GPT-4o, comparing three distinct exploration strategies: direct exploration, standard MCTS, and the proposed SA-MCTS. We report the number of expanded skills.
}
\end{table}

==> tables/memory_ablation.tex <==
% \begin{table}\small
% \centering
% \begin{tabular}{lc}
% \toprule[1.5pt]
% Method & \multicolumn{1}{c}{AndroidWorld$_{SR}$} \\ \midrule
%  Empty &  31.9 \\
% Experience &   \\
% Skill & \\
%  Meta Skill+Skill & 38.8  \\
% \rowcolor[HTML]{E7EEFE}
% Hierarchical Multimodal Skill Module & \textbf{42.2} \\ \bottomrule[1.5pt]
% \end{tabular}
% \caption{\label{abl-memory}
% Ablation experiments in the method of memory.
% }
% \end{table}

\begin{table}\small
\centering
\begin{tabular}{ccc|c}
\toprule[1.5pt]
\multicolumn{3}{c|}{\textbf{Ablation Setting}}     & \multicolumn{1}{c}{\textbf{AndroidWorld}}       \\ \hline
Execution. & Core. & Meta. & SR \\ \hline
& & & 31.9 \\
\checkmark &  &  & 32.7  \\
\checkmark & \checkmark &  & 35.3  \\
& \checkmark    & \checkmark & 38.8 \\
\rowcolor[HTML]{E7EEFE} \checkmark & \checkmark & \checkmark & \textbf{42.2} \\ \bottomrule[1.5pt] \end{tabular}
\caption{\label{abl-memory}
Ablation experiments about the components of HMS. We report task success rate (SR) on AndroidWorld and use \texttt{GPT-4o} + OS-Atlas as the Operator.
}
\end{table}

==> tables/mind2web_live.tex <==


\begin{table}[t]\small
\centering
\resizebox{.98\columnwidth}{!}{
\begin{tabular}{l|lll}
\toprule[1.5pt]
\textbf{Method} & \textbf{Operator} & \textbf{CR} & \textbf{SR} \\ 
\midrule
 & \multicolumn{3}{c}{\textbf{HTML Tree}} \\ \midrule
\multirow{4}{*}{\citeauthor{pan2024webcanvas}}  & GPT-4-Turbo + Choice & 44.3 & 21.1 \\
& GPT-4o + Choice  & 47.6 & 22.1 \\
& Gemini-1.5-Pro + Choice  & 44.6 & 22.3 \\
& GPT-3.5-Turbo + Choice  & 40.2 & 16.5 \\ 
\midrule
& \multicolumn{3}{c}{\textbf{Image}} \\ 
\midrule

\citeauthor{wu2024osatlas} &GPT-4o + OS-Atlas & 50.4$^*$ & 18.4$^*$ \\
\rowcolor[HTML]{E7EEFE}
Mirage-O & GPT-4o + OS-Atlas & \textbf{51.2} & \textbf{21.3}$_{\color{teal}{\textbf{\scriptsize15.8\%}\uparrow}}$ \\ 
\citeauthor{gou2024uground} &GPT-4o + UGround & 50.8$^*$ & 19.2$^*$ \\
\rowcolor[HTML]{E7EEFE}
Mirage-U & GPT-4o + UGround & \textbf{51.4} & \textbf{22.1}$_{\color{teal}{\textbf{\scriptsize15.1\%}\uparrow}}$ \\ 
\citeauthor{yang2024aria-ui} & GPT-4o + Aria-UI & 51.9$^*$ & 22.1$^*$ \\
\rowcolor[HTML]{E7EEFE}
Mirage-A & GPT-4o + Aria-UI & \textbf{53.3} & \textbf{24.0}$_{\color{teal}{\textbf{\scriptsize8.6\%}\uparrow}}$ \\ 
\bottomrule[1.5pt]
\end{tabular}
}
\caption{\label{mind2web_live_result}
Performance comparison on Mind2Web-Live.
We report completion rate (CR) and task success rate (SR). $^*$ means the results are reproduced under the same prompt setting. 
}
\end{table}
